A Simple Approach to Differentiable Rendering of SDFs

We present a simple algorithm for differentiable rendering of surfaces represented by Signed Distance Fields (SDF), which makes it easy to integrate rendering into gradient-based optimization pipelines. To tackle visibility-related derivatives that make rendering non-differentiable, existing physically based differentiable rendering methods often rely on elaborate guiding data structures or reparameterization with a global impact on variance. In this article, we investigate an alternative that embraces nonzero bias in exchange for low variance and architectural simplicity. Our method expands the lower-dimensional boundary integral into a thin band that is easy to sample when the underlying surface is represented by an SDF. We demonstrate the performance and robustness of our formulation in end-to-end inverse rendering tasks, where it obtains results that are competitive with or superior to existing work.

==> 3.methods/4.relation.tex <==
\subsection{Relation to SDF Reparametrization}

Previous works have proposed SDF Reparameterization as a differentiable rendering method tailored for SDFs \cite{Vicini2022sdf, Bangaru2022NeuralSDFReparam}. Here we discuss the relation of our method to it.

At a high level, reparameterization methods work by reparameterizing ray intersection points to follow the motion of the evolving surface. Starting from the rendering equation \eqref{eq:render}, SDF Reparameterization applies a change of variable 
\begin{equation}
    I = \int_{\S} f(T(\w,\theta)) \|DT_\w(u)\times DT_\w(v)\| ~d\w,
\end{equation}
where $T:\S\to\S$ specifies the reparameterization in solid angle space, $DT_\w$ is the differential of $T$ at $\w$, and $\{u, v\}$ is an orthonormal basis of the tangent space at $\w$. Specifically, Vicini et. al. designed their reparameterization to be
\begin{equation}
    \frac{\d}{\d\theta} T(\w,\theta) = \frac{1}{t} \left( \mathbb{I} - \w \cdot \w^\top \right) \v(\x_t, \theta).
\end{equation}
Here $\x_t$ is the weighted average of all intermediate points of sphere tracing. Through a careful design of the weighting, SDF Reparameterization achieves a continuous normal velocity $\v(\x_t)$ from the viewpoint $\x$ (\autoref{fig:sdf_reparam}). This can be seen as interpolating the normal velocities across the visibility discontinuity, which tends to suffer from the drastically different velocities on the two sides of the discontinuity. On the other hand, while our method also requires the normal velocity to evaluate the boundary integral, we relax the discontinuity itself instead of smoothing out the discontinuous normal velocity. As a result, the places that we evaluate the normal vecloity (i.e. the relaxed silhouette points) stay closer to the silhouette, making it a good approximation to the discontinuities. 

% . This can be seen as smoothing out the $0$-th order signal to make the integrand continuous.

% In this way, the integral domain is independent of the changing parameter $\theta$, and one can commute the differential operator and the integration as usual.

% The motions across the visibility discontinuity could change drastically, making SDF Reparameterization vulnerable to distant foreground/background objects, 

% In contrast, our relaxed silhouette points stay very close to the silhouette, making it a good approximation to the discontinuity. 

==> 7.acknowledgement/main.tex <==
\section{acknowledgement}

We would like to thank the entire Mitsuba team for their helpful Github Q\&A support. We are also grateful to Delio Vicini for providing help running SDF Reparameterization, Guandao Yang for sharing his custom Mitsuba integrator for reference, and Yihong Sun for constructive comments on \autoref{fig:intro}.
